Perturbations In Some Dark Energy Models

Dark energy is the candidate that can produce effective negative pressure and make the galaxies and galaxy clusters move away from each other in an accelerated way. The structures of the Universe have evolved from some initial primordial fluctuations and depend on the background dynamics of different components of the Universe like dark matter, dark energy and others. The motivation of this thesis is to investigate how some of the dark energy models manifest themselves in the formation of the structures in the Universe.

==> convension.tex <==
\addcontentsline{toc}{chapter}{Convensions}
\chapter*{Convensions}
%\thispagestyle{plain}
%\null\vfil
%{\noindent\huge\bfseries Convension \par\vspace{10pt}}
%
%\addcontentsline{toc}{chapter}{Convensions}




